SIMS: Simulating Stylized Human-Scene Interactions with Retrieval-Augmented Script Generation

Simulating stylized human-scene interactions (HSI) in physical environments is a challenging yet fascinating task. Prior works emphasize long-term execution but fall short in achieving both diverse style and physical plausibility. To tackle this challenge, we introduce a novel hierarchical framework named SIMS that seamlessly bridges highlevel script-driven intent with a low-level control policy, enabling more expressive and diverse human-scene interactions. Specifically, we employ Large Language Models with Retrieval-Augmented Generation (RAG) to generate coherent and diverse long-form scripts, providing a rich foundation for motion planning. A versatile multicondition physics-based control policy is also developed, which leverages text embeddings from the generated scripts to encode stylistic cues, simultaneously perceiving environmental geometries and accomplishing task goals. By integrating the retrieval-augmented script generation with the multi-condition controller, our approach provides a unified solution for generating stylized HSI motions. We further introduce a comprehensive planning dataset produced by RAG and a stylized motion dataset featuring diverse locomotions and interactions. Extensive experiments demonstrate SIMS's effectiveness in executing various tasks and generalizing across different scenarios, significantly outperforming previous methods.

==> tables/exp_ablation_datasets_hoi.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\resizebox{0.6\linewidth}{!}{%
\begin{tabular}{c|c|c}
\toprule[1.5pt]
\multirow{2}{*}{Datasets} & Success Rate(\%)$\uparrow$ & APD$\uparrow$                                                          \\ 
                          & carry         & carry  \\ \midrule
A                  &                                                                    \\ 
A+VS              &              &                                                       \\ \bottomrule[1.5pt]
\end{tabular}}
\caption{Dataset ablation on HOI Skills}
\label{abl_hoi_data}
\end{table}

==> tables/exp_ablation_datasets_loco.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\resizebox{0.6\linewidth}{!}{%
\begin{tabular}{c|c|c}
\toprule[1.5pt]
\multirow{2}{*}{Datasets} & Success Rate(\%)$\uparrow$ & {APD$\uparrow$}                                                          \\ 
                          & Walk         & Walk  \\ \midrule
100S     &     92.6         &   14.83$\pm$0.35                \\ 
A+100S                  &   95.1     & 14.88$\pm$0.29                               \\ \bottomrule[1.5pt]
\end{tabular}}
\caption{Dataset ablation on Walk Skills}
\label{abl_walk_data}
\end{table}

==> tables/supp_dataset_statistics.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab:dataset_statistics}
\end{table}
